Monitoring with Verified Guarantees

Runtime monitoring is generally considered a light-weight alternative to formal verification. In safety-critical systems, however, the monitor itself is a critical component. For example, if the monitor is responsible for initiating emergency protocols, as proposed in a recent aviation standard, then the safety of the entire system critically depends on guarantees of the correctness of the monitor. In this paper, we present a verification extension to the Lola monitoring language that integrates the efficient specification of the monitor with Hoare-style annotations that guarantee the correctness of the monitor specification. We add two new operators, assume and assert, which specify assumptions of the monitor and expectations on its output, respectively. The validity of the annotations is established by an integrated SMT solver. We report on experience in applying the approach to specifications from the avionics domain, where the annotation with assumptions and assertions has lead to the discovery of safety-critical errors in the specifications. The errors range from incorrect default values in offset computations to complex algorithmic errors that result in unexpected temporal patterns.

==> specifications/contingencies_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
}
\begin{lstlisting}[caption={A simplified Run-Time Assurance \lola specification with three recovery functions for three different flight phases. Assumptions and assertions are used to show that only one recovery function is activated at once.}, label={lst:recovery}]
input alt :  Float32 // Height above ground
input x, y : Float32, Float32 // Position in local coordinate system
input speed : Float32  // Velocity of aircraft
input landing : Bool // Indicates landing mode
input lg_status : (Float32,Float32,FLoat32) // Status of landing gear

// Complex computations
output dst_on_runway $~~~~~$: Float32 := $\sqrt{x^2 + y^2}$
output geofence_violation : Bool $~~$ := ...
output landing_gear_ready : Bool $~~~$:= ...

// Take-off contingency 
output decelerate := alt $<$ 1.0 $\wedge$ speed $<$ 10.0 $\wedge$ dst_on_runway > 20.0 
// In-flight contingency
output parachute := geofence_violation $\wedge$ alt $>$ 100.0 
// Landing contingency
output gain_alt := landing $\wedge$ alt $\ge$ 10.0 $\wedge$ (speed $>$ 10.0 $\vee$
                     !landing_gear_ready[-4..0, true, $\wedge$])
            
// Notifications to the system
trigger decelerate "RECOVERY: Stop take-off by decelerating aircraft."
trigger parachute $~$"RECOVERY: Activate parachute."
trigger gain_alt $~~$"RECOVERY: Gain altitude for next landing attempt."

// By concept of operations: landing is always within geofence.
assume <a1> $\neg$(landing $\wedge$ geofence_violation)
assume <a1> abs(speed) <= 80.0 // Given by data protocol

// Only one contingency is activated at once.
assert <a1> $\neg$( (decelerate $\wedge$ parachute)  $\vee$  (decelerate $\wedge$ gain_alt)
               $\vee$  (parachute  $\wedge$ gain_alt) )  
// Parachute SHALL ONLY be activated 100 m above ground.
assert <a2> parachute $\rightarrow$ alt > 100.0  
\end{lstlisting}


==> specifications/experience/contingency_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:contingency_output}]
input avgDist_laser: Float64 
input actual_laser: Float64
input static_laser: Float64
input avgDist_optical:Float64 
input actual_optical: Float64
input static_optical: Float64
// Assumptions
assume <a1>     avgDist_laser >= 0.0 and actual_laser >= 0.0    
  and static_laser >= 0.0 and avgDist_optical >= 0.0    
  and actual_optical >= 0.0 and static_optical >= 0.0
  and (avgDist_laser + actual_laser + static_laser > 0.0)
  and (avgDist_optical + actual_optical + static_optical > 0.0)
// Trust computations
output rating_laser := 0.2 * static_laser + 0.4 * actual_laser       
     + 0.4 * avgDist_laser
output rating_optical := 0.2 * static_optical + 0.4 * actual_optical + 0.4 * avgDist_optical
output trust_laser := rating_laser / ( rating_laser + rating_optical)
output trust_optical := 1.0 - trust_laser
trigger trust_laser >= 0.5 "Trust in laser"
trigger trust_optical > 0.5 "Trust in optical sensor"
// Assertions
assert <a1> trust_laser $\neq$ trust_optical     
\end{lstlisting}


==> specifications/experience/ctrl_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:ctrl_output}]
import math
input time_s: UInt64
input time_us: UInt64
input vel_x: Float64
input vel_y: Float64
input vel_z: Float64
input fuel: Float64
input power: Float64
input vel_r_x: Float64
input vel_r_y: Float64
input vel_r_z: Float64
// Assumptions
assume <a1>     trace_pos >= 0
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0   
assume<a2>      power > 0.0 
  and power <= power.offset(by: -1).defaults(to: power)  
  and fuel  > 0.0 and fuel  <  fuel.offset(by: -1).defaults(to: fuel + 0.1) 
  and (time_s = time_s.offset(by: -1).defaults(to: 0) 
  and time_us > time_us.offset(by: -1).defaults(to: 0))
  and (time_s > time_s.offset(by: -1).defaults(to: 0) 
       or time_us > time_us.offset(by: -1).defaults(to: 0))
// Frequency computations
output time := cast(time_s) + cast(time_us) / 1000000.0
output start_time := if time.offset(by: -1).defaults(to: -1.0) == -1.0 then time else start_time.offset(by: -1).defaults(to: -1.0) 
output flight_time := time - start_time
output trace_pos @ time_s or time_us or vel_x or vel_y or vel_z or fuel or power or vel_r_x or vel_r_y or vel_r_z := trace_pos.offset(by:-1).defaults(to:-1) + 1
output frequency := 1.0 / ( time - time.offset(by: -1).defaults(to: time - 0.0001) )  // major improvement
output freq_sum := freq_sum.offset(by: -1).defaults(to: 0.0)  + frequency
output freq_avg := freq_sum / cast(trace_pos+1)
output freq_max := if frequency > freq_max.offset(by: -1).defaults(to: frequency)  then frequency else freq_max.offset(by: -1).defaults(to: frequency)
output freq_min := if frequency < freq_min.offset(by: -1).defaults(to: frequency)  then frequency else freq_min.offset(by: -1).defaults(to: frequency)
// Exemplary phase detection
output velocity := sqrt( vel_x*vel_x + vel_y*vel_y + vel_z*vel_z )
output velocity_max := if reset_max.offset(by: -1).defaults(to: false) then velocity else max( velocity, velocity_max.offset(by: -1).defaults(to: 0.0) ) 
output velocity_min := if reset_max.offset(by: -1).defaults(to: false) then velocity else min( velocity, velocity_min.offset(by: -1).defaults(to: 0.0) ) 
output dif_max := abs(velocity_max - velocity_min)
output reset_max := dif_max > 1.0
output reset_time := if reset_max or trace_pos = 0 then time else reset_time.offset(by: -1).defaults(to: 0.0)
output unchanged := if reset_max.offset(by: -1).defaults(to: false) then 0 else unchanged.offset(by: -1).defaults(to: 0) + 1 
trigger unchanged = 150 "Phase detected!"
// Statistics
output vel_dev := abs(vel_r_x-vel_x) + abs(vel_r_y-vel_y) + abs(vel_r_z-vel_z)
output dev_sum := vel_dev + dev_sum.offset(by: -1).defaults(to: 0.0) 
output vel_av := dev_sum / cast((trace_pos+1)*3)
output worst_dev_pos := if worst_dev.offset(by: -1).defaults(to: vel_dev - 1.0) < vel_dev then trace_pos else worst_dev_pos.offset(by: -1).defaults(to: 0) 
output worst_dev := if worst_dev.offset(by: -1).defaults(to: vel_dev - 1.0) < vel_dev then vel_dev else worst_dev.offset(by: -1).defaults(to: 0.0) 
output start_fuel := start_fuel.offset(by: -1).defaults(to: fuel) 
output fuel_level := 1 - ( start_fuel - fuel ) / start_fuel
output fuel_half    := fuel_level < 0.50
output fuel_warning := fuel_level < 0.25
output fuel_danger  := fuel_level < 0.10
output start_power := start_power.offset(by: -1).defaults(to: power) 
output power_p_consumed := ( (start_power - power) / (start_power) )
trigger_once fuel_half    "INFO: Fuel level is half reduced"
trigger_once fuel_warning "WARNING: Fuel level is below 25%"
trigger_once fuel_danger  "DANGER: Fuel level is below 10%"
trigger_once power_p_consumed > 0.50  "Power below half capacity"
trigger_once power_p_consumed > 0.75  "Power below quarter capacity"
trigger_once power_p_consumed > 0.90  "Urgent: Recharge Power!"
// Assertions
assert <a1>     time.offset(by: -1).defaults(to: -1.0) < time  
  and start_time == start_time.offset(by: -1).defaults(to: start_time) 
  and flight_time >= flight_time.offset(by: -1).defaults(to: 0.0)  
assert<a2>      reset_time >= 0.0 
  and start_fuel >= fuel and start_power >= power
  and (!fuel_half.offset(by: -1).defaults(to: false) or fuel_half) 
  and (!fuel_warning.offset(by: -1).defaults(to: false)or fuel_warning)
  and (!fuel_danger.offset(by: -1).defaults(to: false) or fuel_danger) 
  and power_p_consumed >= power_p_consumed.offset(by: -1).defaults(to: power_p_consumed) 
\end{lstlisting}


==> specifications/experience/gps_pos_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:gps_pos_output}]
import math
input lat: Float32
input lon: Float32
input hgt: Float32
input nObjs: UInt64
input nGPSL1: UInt64
input time_s: UInt64
input time_us: UInt64
// Assumptions
assume <a1>     time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0   
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and trace_pos >= 0
// Frequency computations
output time: Float32 := cast(time_s) + cast(time_us) / 1000000.0
output start_time := if time.offset(by: -1).defaults(to: -1.0) == -1.0 then time else start_time.offset(by: -1).defaults(to: -1.0) 
output flight_time := time - start_time
output trace_pos @ lat or lon or hgt or nObjs or nGPSL1 or time_s or time_us := trace_pos.offset(by: -1).defaults(to: -1) + 1 
output frequency := 1.0 / ( time - time.offset(by: -1).defaults(to: time - 0.0001) ) 
output freq_sum := freq_sum.offset(by: -1).defaults(to: 0.0)  + frequency
output freq_avg := freq_sum / cast(trace_pos+1)
output freq_max := if frequency > freq_max.offset(by: -1).defaults(to: 0.0)  then frequency else freq_max.offset(by: -1).defaults(to: 0.0)
output freq_min := if frequency < freq_min.offset(by: -1).defaults(to: 0.0)  then frequency else freq_min.offset(by: -1).defaults(to: 0.0)
// Statistics
output lat_max := if lat > lat_max.offset(by: -1).defaults(to: lat)  then lat else lat_max.offset(by: -1).defaults(to: lat)
output lat_min := if lat < lat_min.offset(by: -1).defaults(to: lat)  then lat else lat_min.offset(by: -1).defaults(to: lat)
output lon_max := if lon > lon_max.offset(by: -1).defaults(to: lon)  then lon else lon_max.offset(by: -1).defaults(to: lon)
output lon_min := if lon < lon_min.offset(by: -1).defaults(to: lon)  then lon else lon_min.offset(by: -1).defaults(to: lon)
output lat_in_bound := max( abs(lat_max), abs(lat_min) ) <= 90.0
output lon_in_bound := max( abs(lon_max), abs(lon_min) ) <= 180.0
trigger !lat_in_bound "Irregular latitude value!"
trigger !lon_in_bound "Irregular longitude value!"
output begin := false
output start_height := if begin.offset(by: -1).defaults(to: true) then hgt else start_height.offset(by: -1).defaults(to: 0.0) 
output hgt_inc_max := max( hgt_inc_max.offset(by: -1).defaults(to: 0.0),  hgt - start_height )
output hgt_dec_max := min( hgt_dec_max.offset(by: -1).defaults(to: 0.0) , hgt - start_height )
trigger hgt_inc_max > 100.0 "Never increase height by more than 100m!"
trigger hgt_dec_max < -100.0 "Never decrease height by more than 100m"
// Assertions
assert <a1>     time.offset(by: -1).defaults(to: -1.0) < time 
  and start_time == start_time.offset(by: -1).defaults(to: start_time) 
  and flight_time >= flight_time.offset(by: -1).defaults(to: 0.0)  
assert <a2>     hgt_inc_max >= 0.0 and hgt_dec_max <= 0.0
  and hgt_inc_max >= hgt_inc_max.offset(by: -1).defaults(to: 0.0) 
  and hgt_dec_max <= hgt_inc_max.offset(by: -1).defaults(to: 0.0) 
  and start_height = start_height.offset(by: -1).defaults(to: start_height)
  and (lat_in_bound.offset(by: -1).defaults(to: true) or !lat_in_bound)   
  and (lon_in_bound.offset(by: -1).defaults(to: true) or !lon_in_bound)   
\end{lstlisting}


==> specifications/experience/gps_vel_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:gps_vel_output}]
input sol_age: Float32
input hor_spd: Float32 
input trk_gnd: Float32
input vert_spd: Float32
input time_s: UInt64
input time_us: UInt64
// Assumptions
assume <a1>     time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0   
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and trace_pos >= 0

assume <a2>     time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0   
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and trace_pos >= 0
// Frequency computations
output time := cast(time_s) + cast(time_us) / 1000000.0
output start_time := if time.offset(by: -1).defaults(to: -1.0) = -1.0 then time else start_time.offset(by: -1).defaults(to: -1.0) 
output flight_time := time - start_time
output trace_pos @ sol_age or hor_spd or  trk_gnd or vert_spd or time_s or time_us := trace_pos.offset(by: -1).defaults(to: -1) + 1
output frequency := 
     1.0 / ( time - time.offset(by: -1).defaults(to: time - 0.0001) )  
output freq_sum := 
     freq_sum.offset(by: -1).defaults(to: 0.0)  + frequency
output freq_avg := freq_sum / cast(trace_pos+1)
output freq_max := if frequency > freq_max.offset(by: -1).defaults(to: frequency)  then frequency else freq_max.offset(by: -1).defaults(to: frequency)
output freq_min := if frequency < freq_min.offset(by: -1).defaults(to: frequency)  then frequency else freq_min.offset(by: -1).defaults(to: frequency)
// Speed computations
output hor_spd_max := if hor_spd > hor_spd_max.offset(by: -1).defaults(to: 0.0)  then hor_spd else hor_spd_max.offset(by: -1).defaults(to: 0.0)
output vert_spd_max := if vert_spd > vert_spd_max.offset(by: -1).defaults(to: 0.0)  then vert_spd else vert_spd_max.offset(by: -1).defaults(to: 0.0)
// Solution age and track over ground (motion direction wrt. north)
trigger sol_age <= 0.5  "Sol age should remain zero!"
output trk_gnd_in_bound := if trk_gnd >= 0.0 and trk_gnd <= 360.0 then trk_gnd_in_bound.offset(by: -1).defaults(to: true)  else  false 
output trk_gnd_max := if trk_gnd > trk_gnd_min.offset(by: -1).defaults(to: 0.0)  then trk_gnd else trk_gnd_min.offset(by: -1).defaults(to: 0.0)
output trk_gnd_min := if trk_gnd < trk_gnd_max.offset(by: -1).defaults(to: 0.0)  then trk_gnd else trk_gnd_max.offset(by: -1).defaults(to: 0.0)
// Assertions
assert <a1> time.offset(by: -1).defaults(to: -1.0) < time  
  and start_time == start_time.offset(by: -1).defaults(to: start_time) 
  and flight_time >= flight_time.offset(by: -1).defaults(to: 0.0)  
assert <a2>     frequency >= 10.0
  and freq_sum >= freq_sum.offset(by: -1).defaults(to: 0.0) + 10.0      
assert <a3> trk_gnd_in_bound.offset(by: -1).defaults(to: true) 
  or !trk_gnd_in_bound 
\end{lstlisting}


==> specifications/experience/health_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}
\tiny
\begin{lstlisting}[label={lst:health_output}]
import math
// average distance to the measured ostacle (range of sight) using laser
input avgDist_laser: Float64    
// average distance to the measured ostacle (range of sight) using camera
input avgDist_optical: Float64  
input vel: Float64
// Assumption
assume <a1>     avgDist_laser <= 100.0 and avgDist_laser >=   0.0   // both in m
  and avgDist_optical <= 50.0  and avgDist_optical >=  0.0   // both in m
  and abs(vel) < 5.5  // in m/s
// Line of sight
output avgDst_dif := min( avgDist_laser, avgDist_optical ) - abs(vel)
trigger avgDst_dif < 5.0 "WARNING: Dynamic Velocity Limit reached"
trigger avgDst_dif < 2.0 "ERROR: Abort mission."
// Assertions
assert <a1>     avgDst_dif < 54.5 and avgDst_dif > -5.5   
\end{lstlisting}


==> specifications/experience/imu_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:imu_output}]
import math
input ax: Float32
input ay: Float32
input az: Float32
input time_s: UInt64
input time_us: UInt64
input counter: Int64
// Assumptions
assume <a1>     time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0   
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and trace_pos >= 0
assume <a2>     ax != ax.offset(by: -1).defaults(to: ax + 0.1)    
  and ay != ay.offset(by: -1).defaults(to: ay + 0.1)
  and az != az.offset(by: -1).defaults(to: az + 0.1) 
// Frequency computations
output time := cast(time_s) + cast(time_us) / 1000000.0
output start_time := if time.offset(by: -1).defaults(to: -1.0) == -1.0 then time else start_time.offset(by: -1).defaults(to: -1.0) 
output flight_time := time - start_time
output trace_pos @ ax or ay or az or time_s or time_us or counter := trace_pos.offset(by: -1).defaults(to: -1) + 1
output frequency := 1.0 / ( time - time.offset(by: -1).defaults(to: time - 0.0001) )  
output freq_sum := freq_sum.offset(by: -1).defaults(to: 0.0)  + frequency
output freq_avg := freq_sum / cast(trace_pos+1)
// Statistics
output deviation := abs( frequency - 100.0)
output exceeds_worst := deviation > worst_dev.offset(by: -1).defaults(to: 0.0) 
output worst_dev_pos := if exceeds_worst then trace_pos else worst_dev_pos.offset(by: -1).defaults(to: 0) 
output worst_dev := if exceeds_worst then deviation else worst_dev.offset(by: -1).defaults(to: 0.0) 
output ax_max := max(abs(ax),ax_max.offset(by:-1).defaults(to:0.0))
output ay_max := max(abs(ay),ay_max.offset(by:-1).defaults(to:0.0))
output az_max := max(abs(az),az_max.offset(by:-1).defaults(to:0.0))
trigger ax > 15.0 or ay > 15.0 or az > 15.0
output frozen_ax := ax.offset(by:-1).defaults(to:0.0) = ax
  and ax.offset(by:-2).defaults(to:0.0)=ax.offset(by:-1).defaults(to:0.0)  
  and ax.offset(by:-3).defaults(to:0.0)=ax.offset(by:-2).defaults(to:0.0)   
  and ax.offset(by:-4).defaults(to:0.0)=ax.offset(by:-3).defaults(to:0.0)  
  and ax.offset(by:-5).defaults(to:0.1)=ax.offset(by:-4).defaults(to:0.0)
output frozen_ay := ay.offset(by:-1).defaults(to:0.0) = ay
  and ay.offset(by:-2).defaults(to:0.0)=ay.offset(by:-1).defaults(to:0.0)  
  and ay.offset(by:-3).defaults(to:0.0)=ay.offset(by:-2).defaults(to:0.0)   
  and ay.offset(by:-4).defaults(to:0.0)=ay.offset(by:-3).defaults(to:0.0)  
  and ay.offset(by:-5).defaults(to:0.1)=ay.offset(by:-4).defaults(to:0.0)
output frozen_az :=  az.offset(by:-1).defaults(to:0.0) = az
  and az.offset(by:-2).defaults(to:0.0)=az.offset(by:-1).defaults(to:0.0)  
  and az.offset(by:-3).defaults(to:0.0)=az.offset(by:-2).defaults(to:0.0)   
  and az.offset(by:-4).defaults(to:0.0)=az.offset(by:-3).defaults(to:0.0)  
  and az.offset(by:-5).defaults(to:0.1)=az.offset(by:-4).defaults(to:0.0)
trigger frozen_ax or frozen_ay or frozen_az
output check_counter := if trace_pos = 0 then false else (counter != (counter.offset(by: -1).defaults(to: -1) + 1) % 100) 
trigger check_counter  "A counter value was ignored."
// Assertions
assert <a1>     time.offset(by: -1).defaults(to: -1.0) < time  
  and start_time == start_time.offset(by: -1).defaults(to: start_time) 
  and flight_time >= flight_time.offset(by: -1).defaults(to: 0.0)  
assert <a2> !frozen_ax and !frozen_ay and !frozen_az
\end{lstlisting}


==> specifications/experience/mm_output_1_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:mm_output_1}]
import math
input stateID_SC: UInt64
// Assumptions
assume<a1>  trace_pos >= 0
// Exemplary state transition analysis
output trace_pos @ stateID_SC := trace_pos.offset(by: -1).defaults(to: -1) + 1
output change_state := if trace_pos = 0 then false 
  else stateID_SC != stateID_SC.offset(by: -1).defaults(to: 0) 
output transitions := if stateID_SC.offset(by:-1).defaults(to: 0) = 0 then stateID_SC == 1 
  else if stateID_SC.offset(by: -1).defaults(to: 0) == 1 then stateID_SC == 1 or stateID_SC == 2
  else if stateID_SC.offset(by: -1).defaults(to: 0) == 2 then stateID_SC == 1 or stateID_SC == 3 
  else if stateID_SC.offset(by: -1).defaults(to: 0) == 3 then stateID_SC == 3
  else false
output invalid_transitions := change_state and !transitions
trigger invalid_transitions "Invalid state transition"
// Assertions
assert <a1> invalid_transitions or
!( stateID_SC.offset(by: -1).defaults(to: 0) != 0 and stateID_SC = 0 )  
assert <a2> (stateID_SC == 1 or stateID_SC == 2 or stateID_SC == 3 )   
  or !( stateID_SC.offset(by: -2).defaults(to: 0) = 1 
   and  transitions.offset(by: -1).defaults(to: false) and transitions )       
\end{lstlisting}


==> specifications/experience/mm_output_2_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:mm_output_2}]
import math
input time_s: UInt64
input time_us: UInt64
input stateID_SC: Int64
input OnGround: UInt64
// Assumptions
assume <a1>     trace_pos >= 0
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0   
assume <a2>     (time_s = time_s.offset(by: -1).defaults(to: 0) 
  and time_us > time_us.offset(by: -1).defaults(to: 0))
  and (time_s > time_s.offset(by: -1).defaults(to: 0) 
       or time_us > time_us.offset(by: -1).defaults(to: 0))
// Frequency computations
output time := cast(time_s) + cast(time_us) / 1000000.0
output start_time := if time.offset(by: -1).defaults(to: -1.0) == -1.0 then time else start_time.offset(by: -1).defaults(to: -1.0) 
output flight_time := time - start_time
output trace_pos @ time_s or time_us or stateID_SC or OnGround := trace_pos.offset(by: -1).defaults(to: -1) + 1
output frequency := 1.0 / ( time - time.offset(by: -1).defaults(to: time - 0.0001) )  
output freq_sum := freq_sum.offset(by: -1).defaults(to: 0.0)  + frequency
output freq_avg := freq_sum / cast(trace_pos+1)
// Phase Statistics
output change_state := if trace_pos = 0 then false 
       else stateID_SC != stateID_SC.offset(by: -1).defaults(to: 0) 
trigger change_state
output entrance_time := if change_state then time 
         else entrance_time.offset(by: -1).defaults(to: time) 
output hover_end := change_state and stateID_SC.offset(by: -1).defaults(to: -1)  = 4
output hover_cur_time := if hover_end then 
time - entrance_time.offset(by: -1).defaults(to: 0.0)else  0.0
output hover_sum_time := hover_sum_time.offset(by: -1).defaults(to: 0.0) + hover_cur_time
output hover_num_times := hover_num_times.offset(by: -1).defaults(to: 0)  + if hover_end then 1 else  0
output hover_max_time := max ( hover_max_time.offset(by: -1).defaults(to: 0.0), hover_cur_time )
output hover_avg_time := if hover_num_times != 0 then hover_sum_time / cast(hover_num_times) else 0.0
output landing_info := if change_state and stateID_SC = 5 then 0.0 else time - entrance_time.offset(by: -1).defaults(to: time) 
output landing_error := stateID_SC = 5 and OnGround != 1 and landing_info > 20.0
// Assertions
assert <a1>     time.offset(by: -1).defaults(to: -1.0) < time 
  and start_time == start_time.offset(by: -1).defaults(to: start_time) 
  and flight_time >= flight_time.offset(by: -1).defaults(to: 0.0)  
assert <a2>     time >= entrance_time and start_time <= entrance_time
  and hover_cur_time >= 0.0 and hover_max_time <= flight_time
assert <a3>     !(landing_error and hover_end) 
  and (!landing_error or landing_info > 0.0)
\end{lstlisting}


==> specifications/experience/nav_output_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:nav_output}]
import math
input lat: Float32
input lon: Float32
input ug: Float32
input vg: Float32
input wg: Float32
input time_s: UInt64
input time_us: UInt64
// Assertion
assume <a1>    trace_pos >= 0   
  and time - time.offset(by: -1).defaults(to: time - 0.1) <= 0.1 
  and time - time.offset(by: -1).defaults(to: time - 0.1) > 0.0 
// Frequency Computation
output time := cast(time_s) + cast(time_us) / 1000000.0
output start_time := if time.offset(by: -1).defaults(to: -1.0) == -1.0 then time else start_time.offset(by: -1).defaults(to: -1.0) 
output flight_time := time - start_time
output trace_pos @lat or lon or ug or vg or wg or time_s or time_us := trace_pos.offset(by: -1).defaults(to: -1) + 1 
output frequency :=  1.0 / ( time - time.offset(by: -1).defaults(to: time - 0.0001) )  
output freq_sum := freq_sum.offset(by: -1).defaults(to: 0.0)  + frequency
output freq_avg := freq_sum / cast(trace_pos+1)
output freq_max := if frequency > freq_max.offset(by: -1).defaults(to: frequency)  then frequency else freq_max.offset(by: -1).defaults(to: frequency)
output freq_min := if frequency < freq_min.offset(by: -1).defaults(to: frequency)  then frequency else freq_min.offset(by: -1).defaults(to: frequency)
// Statistics
output velocity := sqrt( ug*ug + vg*vg + wg*wg)
output lon1_rad := lon.offset(by: -1).defaults(to: 0.0)  * 3.1415926535 / 180.0
output lon2_rad := lon * 3.1415926535 / 180.0
output lat1_rad := lat.offset(by: -1).defaults(to: 0.0)  * 3.1415926535 / 180.0
output lat2_rad := lat * 3.1415926535 / 180.0
output dlon := lon2_rad - lon1_rad
output dlat := lat2_rad - lat1_rad
output a := (sin(dlat/2.0))*(sin(dlat/2.0)) + cos(lat1_rad) * cos(lat2_rad) * (sin(dlon/2.0))*(sin(dlon/2.0))
output x_atan2 := sqrt(a)
output y_atan2 := sqrt(1.0-a)
output c := 2.0 * if x_atan2 > 0.0                     then arctan(y_atan2/x_atan2)
  else if x_atan2 < 0.0 and y_atan2 >= 0.0  
    then arctan(y_atan2/x_atan2) + 3.1415926535
  else if x_atan2 < 0.0 and y_atan2 <  0.0  
    then arctan(y_atan2/x_atan2) - 3.1415926535
  else if x_atan2 = 0.0 and y_atan2 > 0.0   then  3.1415926535 / 2.0
  else if x_atan2 = 0.0 and y_atan2 < 0.0   then -3.1415926535 / 2.0
  else 0.0
output gps_distance := 6373000.0 * c
output passed_time := time - time.offset(by: -1).defaults(to: 0.0) 
output distance_max := velocity * passed_time
output dif_distance := abs( gps_distance - distance_max )  
output detected_jump :=if trace_pos=0 then false else dif_distance>1
trigger detected_jump "Jump!"
// Assertions
assert <a1>     time.offset(by: -1).defaults(to: -1.0) < time  
  and start_time == start_time.offset(by: -1).defaults(to: start_time) 
  and flight_time >= flight_time.offset(by: -1).defaults(to: 0.0) 
assert <a2>   (!detected_jump or gps_distance > distance_max) 
  or (!detected_jump or distance_max > gps_distance)
\end{lstlisting}


==> specifications/experience/tagging_1.tex <==
\lstset
{ %Formatting for code in appendix
    numbers=right,
    stepnumber=1,
    basicstyle=\small,
}

\begin{lstlisting}[label={lst:tagging}]
import math 
input time_s: UInt64
input time_us: UInt64
input vel: Float64
// Assumptions
assume<a1>      (time_s = time_s.offset(by: -1).defaults(to: 0) 
  and time_us > time_us.offset(by: -1).defaults(to: 0))
  and (   time_s > time_s.offset(by: -1).defaults(to: 0) 
       or time_us > time_us.offset(by: -1).defaults(to: 0))
// Exemplary State Statistics
output time := cast(time_s) + cast(time_us) / 1000000.0
output correct_vel := abs( vel ) < 0.3
output cur_state := if correct_vel then
  if cur_state.offset(by: -1).defaults(to: 0) = 0 then 1 else 2 else 0                  
output start_interval := cur_state = 2 
output interval_start := if start_interval then interval_start.offset(by: -1).defaults(to: 0.0) else time
trigger start_interval "Interval started!"
output end_interval := cur_state.offset(by: -1).defaults(to: 0)  > 0 and !correct_vel and time_since_start >  5.0
trigger end_interval "Interval ended!"
output time_since_start := time - interval_start.offset(by: -1).defaults(to: 0.0) 
// Assertions
assert <a1>     !(start_interval and end_interval) 
  and time_since_start > 0.0
\end{lstlisting}

